Designing Multi-Commodity Flow Trees

The traditional multi-commodity flow problem assumes a given flow network in which multiple commodities are to be maximally routed in response to given demands. This paper considers the multi-commodity flow network-design problem: given a set of multi-commodity flow demands, find a network subject to certain constraints such that the commodities can be maximally routed. This paper focuses on the case when the network is required to be a tree. The main result is an approximation algorithm for the case when the tree is required to be of constant degree. The algorithm reduces the problem to the minimum-weight balanced-separator problem; the performance guarantee of the algorithm is within a factor of 4 of the performance guarantee of the balanced-separator procedure. If Leighton and Rao's balanced-separator procedure is used, the performance guarantee is O(log n). This improves the O(log^2 n) approximation factor that is trivial to obtain by a direct application of the balanced-separator method.

==> ipl-ex1.tex <==
\begin{picture}(0,0)%
\special{psfile=ex1a.ps}%
\end{picture}%
\setlength{\unitlength}{0.012500in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(457,248)(126,561)
\put(220,772){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$f_1$}}}
\put(480,700){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$(b)$}}}
\put(424,787){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$A_{1}$}}}
\put(423,737){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$A_{2}$}}}
\put(539,787){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$B_{1}$}}}
\put(539,737){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$B_{2}$}}}
\put(434,762){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$f_2$}}}
\put(548,762){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$f_3$}}}
\put(218,702){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$(a)$}}}
\put(205,561){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$(c)$}}}
\put(483,564){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$(d)$}}}
\put(159,767){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$A$}}}
\put(280,766){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$B$}}}
\end{picture}




==> ipl-ex2.tex <==
\begin{picture}(0,0)%
\special{psfile=ex2a.ps}%
\end{picture}%
\setlength{\unitlength}{0.012500in}%
%
\begingroup\makeatletter\ifx\SetFigFont\undefined
% extract first six characters in \fmtname
\def\x#1#2#3#4#5#6#7\relax{\def\x{#1#2#3#4#5#6}}%
\expandafter\x\fmtname xxxxxx\relax \def\y{splain}%
\ifx\x\y   % LaTeX or SliTeX?
\gdef\SetFigFont#1#2#3{%
  \ifnum #1<17\tiny\else \ifnum #1<20\small\else
  \ifnum #1<24\normalsize\else \ifnum #1<29\large\else
  \ifnum #1<34\Large\else \ifnum #1<41\LARGE\else
     \huge\fi\fi\fi\fi\fi\fi
  \csname #3\endcsname}%
\else
\gdef\SetFigFont#1#2#3{\begingroup
  \count@#1\relax \ifnum 25<\count@\count@25\fi
  \def\x{\endgroup\@setsize\SetFigFont{#2pt}}%
  \expandafter\x
    \csname \romannumeral\the\count@ pt\expandafter\endcsname
    \csname @\romannumeral\the\count@ pt\endcsname
  \csname #3\endcsname}%
\fi
\fi\endgroup
\begin{picture}(276,211)(317,542)
\put(408,603){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$S_1$}}}
\put(495,673){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$L_2$}}}
\put(494,600){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$S_2$}}}
\put(317,683){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$S$}}}
\put(411,672){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$L_1$}}}
\put(477,738){\makebox(0,0)[lb]{\smash{\SetFigFont{12}{14.4}{rm}$L$}}}
\end{picture}



